Narrow Proofs May Be Maximally Long

We prove that there are 3-CNF formulas over n variables that can be refuted in resolution in width w but require resolution proofs of size n^Omega(w). This shows that the simple counting argument that any formula refutable in width w must have a proof in size n^O(w) is essentially tight. Moreover, our lower bound generalizes to polynomial calculus resolution (PCR) and Sherali-Adams, implying that the corresponding size upper bounds in terms of degree and rank are tight as well. Our results do not extend all the way to Lasserre, however, where the formulas we study have proofs of constant rank and size polynomial in both n and w.

==> defs-proofcplx11.tex <==
%
% SOME NOTATION FOR THE PROOF COMPLEXITY COURSE 2011/12 
%
% (This file should be included after the other macro files since it
% redefines some of these macros.)
%

% Default "line" in proof
\newcommand{\linestd}{L}

% Default notation for space (as quantity)
\newcommand{\spacestd}{s}

% Default "bit" or "truth value"
\renewcommand{\truthval}{\nu}
\renewcommand{\truthvalalt}{\mu}
\renewcommand{\truthval}{b}
\renewcommand{\truthvalalt}{c}


% Some experimental stuff for formatting of "standard" proof systems
%
% BEGIN experimental stuff
%
\DeclareFontFamily{OT1}{pzc}{}
\DeclareFontShape{OT1}{pzc}{m}{it}{<-> s * [1.200] pzcmi7t}{}
\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}

\renewcommand{\proofsystemformat}[1]{\scriptscriptstyle{\mathpzc{#1}}}
%    \renewcommand{\proofsystemformat}[1]{\mathfrak{#1}}
%    \newcommand{\proofsystemformat}[1]{\mathsf{#1}}

% END experimental stuff

%
% PROBABLY THE ABOVE SHOULD BE CHANGED TO:
%
%    \renewcommand{\proofsystemformat}[1]{\scriptscriptstyle{\mathcal{#1}}}
%
% AND THEN ONE COULD HAVE COMMANDS LIKE:
%
%    \newcommand{\proofsystemtextformat}[1]{\scriptscriptstyle{\mathcal{#1}}}
%    \newcommand{\restext}{\proofsystemtextformat{R}}
%    \newcommand{\treerestext}{\proofsystemtextformat{T}}
%    \newcommand{\pctext}{\proofsystemtextformat{PC}}
%    \newcommand{\pcrtext}{\proofsystemtextformat{PCR}}
%    \newcommand{\cptext}{\proofsystemtextformat{CP}}
%    
% FOR REFERRING TO THE PROOF SYSTEMS IN RUNNING TEXT
%

%
% NOTATION FOR RESOLUTION, PC, PCR AND CP
%
\renewcommand{\resnot}{\proofsystemformat{R}}
\renewcommand{\treeresnot}{\proofsystemformat{T}}
\renewcommand{\pcnot}{\proofsystemformat{PC}}
\renewcommand{\pcrnot}{\proofsystemformat{PCR}}
\newcommand{\cpnot}{\proofsystemformat{CP}}

%    \renewcommand{\prsyststd}{\mathcal{P}}
% Standard proof system in running text
\renewcommand{\prsyststd}{\mathpzc{P}}
\renewcommand{\psstd}{\prsyststd}
% Standard proof system in math subscript
\newcommand{\psstdsub}{\proofsystemformat{P}}



%
% NOTATION FOR PROOF COMPLEXITY MEASURES
%

% New notation for the empty clause and for measures of refuting formulas
\renewcommand{\emptycl}{\bot}

\renewcommand{\refutabbrev}[1]{\derivabbrev{#1}{\!\bot}}
\renewcommand{\refutabbrevsmall}[1]{\derivabbrevsmall{#1}{\!\bot}}
\renewcommand{\refutabbrevcompact}[1]{\derivabbrevcompact{#1}{\!\bot}}

\renewcommand{\refof}[2]{\derivof{#1}{#2}{\bot}}

% Macros for monomial space measures
\newcommand{\mspacestd}{{\spacestd}}
\newcommand{\mspaceof}[2][]{\genericformsmall{Sp_{#1}}{#2}}
\newcommand{\Mspaceof}[2][]{\genericformcompact{Sp_{#1}}{#2}}
\newcommand{\mspaceref}[2][]{\genericrefsmall{Sp}{#1}{#2}}
\newcommand{\Mspaceref}[2][]{\genericrefcompact{Sp}{#1}{#2}}
\newcommand{\mspacederiv}[3][]{\genericderivsmall{Sp}{#1}{#2}{#3}}
\newcommand{\Mspacederiv}[3][]{\genericderivcompact{Sp}{#1}{#2}{#3}}

% Macros for degree measures
\newcommand{\mdegreestd}{{\spacestd}}
\newcommand{\mdegreeof}[2][]{\genericformsmall{Deg_{#1}}{#2}}
\newcommand{\Mdegreeof}[2][]{\genericformcompact{Deg_{#1}}{#2}}
\newcommand{\mdegreeref}[2][]{\genericrefsmall{Deg}{#1}{#2}}
\newcommand{\Mdegreeref}[2][]{\genericrefcompact{Deg}{#1}{#2}}
\newcommand{\mdegreederiv}[3][]{\genericderivsmall{Deg}{#1}{#2}{#3}}
\newcommand{\Mdegreederiv}[3][]{\genericderivcompact{Deg}{#1}{#2}{#3}}

% Polynomial calculus configurations
\newcommand{\pcconf}{\clausesetformat{P}}


%
% New asymptotic notation
%

\newcommand{\BIGOHTILDE}[1]{\mathrm{\tilde{O}} \left( #1 \right)}
\newcommand{\Bigohtilde}[1]{\mathrm{\tilde{O}} \bigl( #1 \bigr)}
\newcommand{\bigohtilde}[1]{\mathrm{\tilde{O}} ( #1 )}


%
% TRY OUT NEW NOTATION FOR SOME FORMULA FAMILIES
%

%
% PHP formulas
%
\renewcommand{\PHPnot}[2]{\formulaformat{PHP}^{#1}_{#2}}
\renewcommand{\extPHPnot}[2]%
    {\ephpnot{#1}{#2}}
%        {\extendedversion{\formulaformat{PHP}}^{#1}_{#2}}

\renewcommand{\phpnot}[2]{\formulaformat{PHP}^{#1}_{#2}}
\newcommand{\ephpnot}[2]%
    {\vphantom{\extendedversion{\formulaformat{PHP}}}
      {\smash{\extendedversion{\formulaformat{PHP}}}
        \vphantom{\formulaformat{PHP}}}^{#1}_{#2}}

\newcommand{\fphpnot}[2]{\formulaformat{FPHP}^{#1}_{#2}}
\newcommand{\efphpnot}[2]%
    {\vphantom{\extendedversion{\formulaformat{FPHP}}}
      {\smash{\extendedversion{\formulaformat{FPHP}}}
        \vphantom{\formulaformat{FPHP}}}^{#1}_{#2}}

\newcommand{\ontophpnot}[2]%
    {\formulaformat{Onto}\text{-}\formulaformat{PHP}^{#1}_{#2}}

\newcommand{\ontofphpnot}[2]%
    {\formulaformat{Onto}\text{-}\formulaformat{FPHP}^{#1}_{#2}}

% The "bit-version" of the PHP formula claiming that there are n+1 distinct
% strings of length log n
\newcommand{\bphpnot}[2]{\formulaformat{BPHP}^{#1}_{#2}}

\renewcommand{\GraphPHPnot}[1][G]{\formulaformat{PHP}({#1})}
\renewcommand{\GraphFPHPnot}[1][G]{\formulaformat{FPHP}({#1})}
\renewcommand{\graphphpnot}[1][G]{\GraphPHPnot[#1]}
\renewcommand{\graphfphpnot}[1][G]{\GraphFPHPnot[#1]}

%
% Tseitin formulas
%

\renewcommand{\tseitinnot}[2]{\formulaformat{Ts}({#1,#2})}
\renewcommand{\tseitinparity}[2]{\ensuremath{\formulaformat{PARITY}_{#1,#2}}}

%
% Ordering principle formulas
%

\newcommand{\popnot}[1]{\formulaformat{POP}_{#1}}
\newcommand{\epopnot}[1]%
    {\extendedversion{\formulaformat{POP}}_{#1}}
\newcommand{\lopnot}[1]{\formulaformat{LOP}_{#1}}
\newcommand{\elopnot}[1]%
    {\extendedversion{\formulaformat{LOP}}_{#1}}


%
% NOTATION FOR [PD11]
%

\newcommand{\unitderives}{\vdash_1}
\newcommand{\decseq}{\Delta}


%
% NOTATION FOR NEW PCR SPACE LOWER BOUND
%

% square brackets [#1]
\providecommand{\numset}[1]{[#1]}
% the set {0,...,n-1}
\providecommand{\zeronumset}[1]{[0,#1)}
% domain
\DeclareMathOperator{\dom}{dom}
% The value of a function (2nd parameter) under an assignment (1st parameter)
\providecommand{\fnval}[2]{#1(#2)}
% an assignment (on the left) satisfies a commitment (on the right)
\providecommand{\VAsatisfies}{\vDash}
% an index variable (#1: variable, #2: index)
\providecommand{\varix}[2]{#1[#2]} % was: #1_{#2}

% number of bits needed to code a hole when there are n holes (log_2 n)
\providecommand{\logn}{\ell}
% commitment sets
%    \providecommand{\aA}{\mathbb{A}}
%    \providecommand{\bB}{\mathbb{B}}
\providecommand{\aA}{\mathcal{A}}
\providecommand{\bB}{\mathcal{B}}
% single commitment
\providecommand{\cC}{C}
% set of all monomials
\providecommand{\allM}{M}
% single monomial
\providecommand{\oneM}{m}
% Gamma set in magic lemma
\providecommand{\gGamma}{\Gamma}
% set used to prove Hall's theorem in magic lemma
\providecommand{\otherset}{S}
% configuration
\providecommand{\pP}{\mathbb{P}}
% assignments
\providecommand{\vV}{\alpha}
\providecommand{\wW}{\beta}
% neighborhood of a set in graph constructed in magic lemma
\providecommand{\neigh}{N}
% matchings constructed in magic lemma
\providecommand{\match}{f}
% polynomial inferred during a PCR proof
\providecommand{\poly}{P}
% a pigeonhole axiom
\providecommand{\paxiom}{D}


%
% SOME PEBBLING-RELATED STUFF
%

% Sources and sinks of DAG
\newcommand{\sourcestd}{s}
\newcommand{\sinkstd}{z}
\newcommand{\sourcesetstd}{S}
\newcommand{\sinksetstd}{Z}
\newcommand{\sourcesof}[1]{S({#1})}
\newcommand{\sinksof}[1]{Z({#1})}


%
% NOTATION AND TERMINOLOGY FOR "PROJECTED CLAUSES" USED TO PROVE
% TIME SPACE TRADE-OFFS FOR RESOLUTION
%

\newcommand{\varvecx}{\varvec{\varx}}
\newcommand{\varvecy}{\varvec{\vary}}
\newcommand{\varvecz}{\varvec{\varz}}

\newcommand{\varsdary}[2]{\setsofvarsorlitsup{Vars}{#1}{#2}}

\newcommand{\farity}{d}
\newcommand{\ff}[1][]{f_{#1}}
\newcommand{\fg}[1][]{g_{#1}}
\newcommand{\ffd}{\ff[\farity]}

\newcommand{\signedfunc}[3][\ff]{#1^{#2}({#3})}
\newcommand{\signedfuncnoarg}[2][\ff]{#1^{#2}}

\newcommand{\anfprojsubst}[1][\funcpebc]{an \mbox{${#1}$-pro}\-jec\-tion\xspace}
\newcommand{\fprojsubst}[1][\funcpebc]{\mbox{${#1}$-pro}\-jec\-tion\xspace}

\newcommand{\spacerespecting}{space-faithful\xspace}
\newcommand{\Spacerespecting}{Space-faithful\xspace}
\newcommand{\SPACERESPECTING}{Space-Faithful\xspace}
%    \newcommand{\spacerespecting}{space-respecting\xspace}
%    \newcommand{\Spacerespecting}{Space-respecting\xspace}
%    \newcommand{\SPACERESPECTING}{Space-Respecting\xspace}

\newcommand{\sprdeg}{K}

% Projected clauses: terminology
\newcommand{\projectionsubst}{projection\xspace}
\newcommand{\projectverb}{project\xspace}
\newcommand{\projectingverb}{projecting\xspace}
\newcommand{\projectedverb}{projected\xspace}
\newcommand{\projectsverb}{projects\xspace}
\newcommand{\Projectionsubst}{Projection\xspace}
\newcommand{\Projectverb}{Project\xspace}
\newcommand{\Projectedverb}{Projected\xspace}
\newcommand{\Projectsverb}{Projects\xspace}


% Projected clauses, generic notation
% \projcl[projected down on which formula]{clause set being projected}
\newcommand{\projclnot}[1][\funcpebc]{{\formatfunctiontoset{proj}\!}_{#1}}
\newcommand{\projcl}[2][\funcpebc]{{\formatfunctiontoset{proj}\!}_{#1}({#2})}
\newcommand{\localprojclnot}[1][\funcpebc]{{\formatfunctiontoset{proj}\!}^{\,L}_{#1}}
\newcommand{\localprojcl}[2][\funcpebc]{{\formatfunctiontoset{proj}\!}^{\,L}_{#1}({#2})}

% Projection for resolution-based proof systems
% \projcl[projected down on which formula]{clause set being projected}
\newcommand{\rprojclnot}[1][\funcpebc]{{\formatfunctiontoset{Rproj}\!}_{#1}}
\newcommand{\rprojcl}[2][\funcpebc]{{\formatfunctiontoset{Rproj}\!}_{#1}({#2})}
\newcommand{\localrprojclnot}[1][\funcpebc]{{\formatfunctiontoset{Rproj}\!}^{\,L}_{#1}}
\newcommand{\localrprojcl}[2][\funcpebc]{{\formatfunctiontoset{Rproj}\!}^{\,L}_{#1}({#2})}


% \Lorspecfuncproj[pebbling degree]{variable}{clause}{function}
% \Lorspecnotfuncproj[pebbling degree]{variable}{clause}{function}
% \witnessproj[function]{pos lit}{neg lit}{clause}
%
\newcommand{\Lorspecfuncproj}[4][\pebdeg]%
    {\Lor_{{#2} \in \clpospart{#3}} \specfuncwithvecarg[#1]{#4}{#2}}    
\newcommand{\Lorspecnotfuncproj}[4][\pebdeg]%
    {\Lor_{\olnot{#2} \in \clnegpart{#3}} \specnotfuncwithvecarg[#1]{#4}{#2}}
\newcommand{\witnessproj}[4][\funcpebc]%	   
    {\Lorspecfuncproj{#2}{#4}{#1} \lor \Lorspecnotfuncproj{#3}{#4}{#1}}

\newcommand{\Lorspecfuncprojnodisplay}[4][\pebdeg]%
    {\Lornodisplay_{{#2} \in \clpospart{#3}} \specfuncwithvecarg[#1]{#4}{#2}}    
\newcommand{\Lorspecnotfuncprojnodisplay}[4][\pebdeg]%
    {\Lornodisplay_{\olnot{#2} \in \clnegpart{#3}} \specnotfuncwithvecarg[#1]{#4}{#2}}
\newcommand{\witnessprojnodisplay}[4][\funcpebc]%	   
    {\Lorspecfuncprojnodisplay{#2}{#4}{#1} \lor \Lorspecnotfuncprojnodisplay{#3}{#4}{#1}}

%
% NOTATION FOR GENERALIZED PEBBLING CONTRADICTIONS
%

%     \pebcontrwithfunc[graph]{degree}{function}
\newcommand{\pebcontrwithfunc}[3][G]{\formulaformat{Peb}^{#2}_{#1}[{#3}]}

% WARNING This ``3-cnf-version-via-tilde'' macro might not work well in displayed mode
\newcommand{\extendedpebcontrwithfunc}[3][G]%
    {{\vphantom{\formulaformat{Peb}}\smash{\extendedversion{\formulaformat{Peb}}}}^{#2}_{#1}[{#3}]}
%    \newcommand{\extendedpebcontrwithfunc}[3][G]%
%        {\extendedversion{\formulaformat{Peb}}^{#2}_{#1}[{#3}]}


% Generic pebbling contradiction with default Boolean function 
% (defined below) assumed as function
%     \genericpebcontr[graph]{degree}
\newcommand{\genericpebcontr}[2][G]{\pebcontrwithfunc[#1]{#2}{\funcpebc}}

% Analogous commands for pebbling formulas, i.e., target axioms removed
\newcommand{\pebcontrwithfuncNT}[3][G]%
     {\dummystar\!\!\formulaformat{Peb}^{#2}_{#1}[{#3}]}
\newcommand{\genericpebcontrNT}[2][G]%
     {\pebcontrwithfuncNT[#1]{#2}{\funcpebc}}

% Default Boolean function used in generalized pebbling contradictions
%     \funcpebc[degree] ; default is subindex being empty
\newcommand{\funcpebc}[1][]{f_{#1}}
\newcommand{\notfuncpebc}[1][]{\lnot f_{#1}}

%
% NOTATION FOR ``CANONICAL REPRESENTATIONS'' OF FUNCTIONS AS CNFs
%

%     \clfunc{function}{applied on vars of which vertex}{pebbling degree}
%     \clnotfunc is representation of negated function
\newcommand{\clausesreprfunction}{\formatfunctiontoset{Cl}}
\newcommand{\clfunc}[3]{\clausesreprfunction[{#1}_{{#3}}({\varvec{#2}})]}
\newcommand{\clnotfunc}[3]{\clausesreprfunction[\lnot{#1}_{{#3}}({\varvec{#2}})]}
%     \clfuncstd[function, default assumed]{vertex}
\newcommand{\clfuncstd}[2][\funcpebc]{\clfunc{#1}{#2}{\pebdeg}}
\newcommand{\clnotfuncstd}[2][\funcpebc]{\clnotfunc{#1}{#2}{\pebdeg}}

%
% NOTATION FOR THE BOOLEAN FUNCTIONS THEMSELVES
%

\newcommand{\varvec}[1]{\vec{#1}}

% Writing out the function as taking a vector 
%     \specfuncwithvecarg[degree]{function}{vertex}
%     \specnotfuncwithvecarg is same thing for negated function
\newcommand{\specfuncwithvecarg}[3][\pebdeg]%
	   {{#2}_{#1}(\varvec{#3})}
\newcommand{\specnotfuncwithvecarg}[3][\pebdeg]%
	   {\lnot {#2}_{#1}(\varvec{#3})}

%     \funcwithvecarg is same thing, except assuming default function
\newcommand{\funcwithvecarg}[2][\pebdeg]%
           {\specfuncwithvecarg[{#1}]{\funcpebc}{#2}}
\newcommand{\notfuncwithvecarg}[2][\pebdeg]%
           {\specnotfuncwithvecarg[{#1}]{\funcpebc}{#2}}

%     \funcwithvecargstd assumes also standard vertex v
\newcommand{\funcwithvecargstd}%
	   {\funcwithvecarg[\pebdeg]{v}}
\newcommand{\notfuncwithvecargstd}%
	   {\notfuncwithvecarg[\pebdeg]{v}}

% Writing out the function as taking d arguments v_1, ..., v_d
%     \specfuncwithargspebcontr[degree]{function}{vertex}
%     \specnotfuncwithargspebcontr is same thing for negated function
\newcommand{\specfuncwithargspebcontr}[3][\pebdeg]%
	   {{#2}_{#1}({#3}_1, \ldots, {#3}_{\pebdeg})}
\newcommand{\specnotfuncwithargspebcontr}[3][\pebdeg]%
	   {\lnot {#2}_{#1}({#3}_1, \ldots, {#3}_{\pebdeg})}

%     \funcwithargspebcontr is same thing, except assuming default function
\newcommand{\funcwithargspebcontr}[2][\pebdeg]%
	   {{\funcpebc}_{#1}({#2}_1, \ldots, {#2}_{\pebdeg})}
\newcommand{\notfuncwithargspebcontr}[2][\pebdeg]%
	   {\lnot {\funcpebc}_{#1}({#2}_1, \ldots, {#2}_{\pebdeg})}

%     \funcwithargspebcontrstd assumes also standard vertex v
\newcommand{\funcwithargspebcontrstd}%
	   {\funcwithargspebcontr[\pebdeg]{v}}
\newcommand{\notfuncwithargspebcontrstd}%
	   {\notfuncwithargspebcontr[\pebdeg]{v}}

%
% NOTATION FOR ``SUBSTITUTION FORMULAS''
%

\newcommand{\clpospart}[1]{#1^{+}}
\newcommand{\clnegpart}[1]{#1^{-}}
%    \newcommand{\clpospart}[1]{{#1}^{+}}
%    \newcommand{\clnegpart}[1]{{#1}^{-}}


% Substitution formula
% \substform{CNF formula}{Boolean function}
\newcommand{\substform}[2]{{#1}[{#2}]}
\newcommand{\Substform}[2]{{#1}\bigl[{#2}\bigr]}

\newcommand{\substformtext}{substitution formula\xspace}
\newcommand{\Substformtext}{Substitution formula\xspace}
\newcommand{\SUBSTFORMTEXT}{Substitution Formula\xspace}

\newcommand{\fsubsttext}[1][{\funcpebc[\pebdeg]}]%
    {${#1}$-substitution\xspace}
\newcommand{\substformtextwithargs}[2]{\fsubsttext[#1] of ${#2}$\xspace}
%
% NOTATION & TERMINOLOGY FOR BOOLEAN FUNCTIONS USED IN PEBBL CONTRADICTIONS
%

% ``Non-authoritarian'' function
\newcommand{\authoritarian}{authoritarian\xspace}
\newcommand{\Authoritarian}{Authoritarian\xspace}
\newcommand{\nonauthoritarian}{non-authoritarian\xspace}
\newcommand{\Nonauthoritarian}{Non-authoritarian\xspace}

% Notation for standard or-pebbling contradiction
\newcommand{\orpebcontr}[2][G]{\pebcontrwithfunc[#1]{#2}{\lor}}
\newcommand{\orpebpyramidcontr}[2][]{\orpebcontr[\Pi_{#1}]{#2}}

\newcommand{\orpebcontrtext}{OR-pebbling contradiction\xspace}

% Notation for threshold k-true-variables-out-of-d function
% \ntrues is default parameter for number of true variables k
\newcommand{\ntrues}{k}
%    \ktrue[out of d, omitted by default]{# true variables}
\newcommand{\ktrue}[2][]{{\mathit{thr}}_{#1}^{#2}}
%%%% \newcommand{\ktrue}[2][]{{#2}\text{\textit{-true}}_{#1}}
% Standard notation for k-true-out-of-d
\newcommand{\ktruestd}[1][]{\ktrue[#1]{\ntrues}}
% Notation for k-true-out-of-d when also specifying parameter variables
\newcommand{\ktruewithargs}[2]%
    {\ktrue[\pebdeg]{#1}({#2}_1, \ldots, {#2}_{\pebdeg})}

% Notation and name for k-out-of-d pebbling contradictions
\newcommand{\ktruepebcontr}[2][G]{\pebcontrwithfunc[#1]{#2}{\ktruestd{}}}
\newcommand{\ktruepebcontrtext}[1][\ntrues]%
    {${#1}$-true-pebbling contradiction\xspace}

% Notation and terminology for XOR-pebbling contradictions
\newcommand{\xorpebcontrtext}{XOR-pebbling contradiction\xspace}

\newcommand{\xorpebcontr}[2][G]{\pebcontrwithfunc[#1]{#2}{\xor}}
\newcommand{\xorbinarypebcontr}[2][G]{\pebcontrwithfunc[#1]{#2}{\xor_2}}

%Notation for the XOR function itself
\renewcommand{\xor}{\oplus}
\newcommand{\Xor}{{\textstyle \bigoplus}}

% ``Witness clauses'' for XOR function for individual vertices
\newcommand{\xorvertex}[3][\pebdeg]{\Xor_{{#3}=1}^{#1} {#2}_{#3}}
\newcommand{\notxorvertex}[3][\pebdeg]{\lnot \Xor_{{#3}=1}^{#1} {#2}_{#3}}

% Complete ``witness clauses'' for sets of black and white pebbles for 
% XOR-pebbling contradictions
\newcommand{\Lornotxor}[3][i]%
    {\Lor_{{#2} \in {#3}}\notxorvertex{#2}{#1}}
\newcommand{\Lorxor}[3][i]%
    {\Lor_{{#2} \in {#3}}\xorvertex{#2}{#1}}


\ifthenelse{\isundefined{\DONOTUSEMETACOMMENTS}}
{
%
% "META COMMENTS" TO BE TOGGLED ON OR OFF (FOR COMMENTS DURING WRITE-UP)
%

\newtheoremstyle{metacommenttheoremstyle}% name
    {3pt}%      Space above
    {3pt}%      Space below
    {\sffamily \itshape \scriptsize
      % or  \footnotesize or \small
    }%         Body font
    {}%         Indent amount (empty = no indent, \parindent = para indent)
    {\bfseries \scshape \footnotesize }% Thm head font
    {:}%        Punctuation after thm head
    { }%     Space after thm head: " " = normal interword space;
    %       \newline = linebreak
    {}%         Thm head spec (can be left empty, meaning `normal')
    
\theoremstyle{metacommenttheoremstyle}

\newtheorem{jncommentcontainer}{Jakob's comment}
          

\ifthenelse{\isundefined{\DONOTINSERTCOMMENTS}}
{ % Turn comments ON
  \newcommand{\jncomment}[1]%
  {\begin{jncommentcontainer} \textcolor{blue}{#1} \end{jncommentcontainer}}
}
{ % Turn comments OFF
  \newcommand{\jncomment}[1]{}
}
}
{}




==> editingmacros.tex <==
%
% MACROS SPECIFIC TO "META FORMATTING" OF CURRENT PAPER
%=======================================================
%

% Massimo <2013-10-20 Sun>
% Use more colors in order to make comments more readable
\RequirePackage[usenames,dvipsnames]{color}

%
% HOW TO REFER TO THE AUTHORS
%

\newcommand{\theauthorAA}{the first author\xspace}
\newcommand{\TheauthorAA}{The first author\xspace}

\newcommand{\theauthorML}{the second author\xspace}
\newcommand{\TheauthorML}{The second author\xspace}

\newcommand{\theauthorJN}{the third author\xspace}
\newcommand{\TheauthorJN}{The third author\xspace}

%
% SWITCHING BETWEEN APPENDIX AND SECTION REFERENCES
%
% \refsecapp is defined to make it easy to change appendix references in
% the submission into section references in the full paper.
%


\ifthenelse{\boolean{conferenceversion}}
{
  % Version of commands for extended abstract with appendices
  \newcommand{\refsecapp}[1]{Appendix~\ref{#1}}
  \newcommand{\Refsecapp}[1]{Appendix~\ref{#1}}
  \newcommand{\reftwosecapps}[2]{Appendices~\ref{#1} and~\ref{#2}}
  \newcommand{\Reftwosecapps}[2]{Appendices~\ref{#1} and~\ref{#2}}
  \newcommand{\Sectionappendixtext}{Appendix\xspace}
  \newcommand{\sectionappendixtext}{appendix\xspace}
  \newcommand{\Sectionsappendicestext}{Appendices\xspace}
  \newcommand{\sectionsappendicestext}{appendices\xspace}
}
{
  % Version of commands for full-length paper
 \newcommand{\refsecapp}[1]{Section~\ref{#1}}
 \newcommand{\Refsecapp}[1]{Section~\ref{#1}}
 \newcommand{\reftwosecapps}[2]{Sections~\ref{#1} and~\ref{#2}}
 \newcommand{\Reftwosecapps}[2]{Sections~\ref{#1} and~\ref{#2}}
 \newcommand{\Sectionappendixtext}{Section\xspace}
 \newcommand{\sectionappendixtext}{section\xspace}
 \newcommand{\Sectionsappendicestext}{Sections\xspace}
 \newcommand{\sectionsappendicestext}{sections\xspace}
}

%
% "META COMMENTS" TO BE TOGGLED ON OR OFF (FOR COMMENTS DURING WRITE-UP)
%

\newtheoremstyle{metacommenttheoremstyle}% name
    {3pt}%      Space above
    {3pt}%      Space below
    {\sffamily \itshape \scriptsize
      % or  \footnotesize or \small
    }%         Body font
    {}%         Indent amount (empty = no indent, \parindent = para indent)
    {\bfseries \scshape \footnotesize }% Thm head font
    {:}%        Punctuation after thm head
    { }%     Space after thm head: " " = normal interword space;
    %       \newline = linebreak
    {}%         Thm head spec (can be left empty, meaning `normal')

\theoremstyle{metacommenttheoremstyle}

\newtheorem{aacommentcontainer}{Albert's comment}
\newtheorem{mlcommentcontainer}{Massimo's comment}
\newtheorem{jncommentcontainer}{Jakob's comment}


\ifthenelse{\isundefined{\DONOTINSERTCOMMENTS}}
{ % Turn comments ON
  \newcommand{\aacomment}[1]%
  {\begin{aacommentcontainer} \textcolor{red}{#1} \end{aacommentcontainer}}

  \newcommand{\mlcomment}[1]%
  {\begin{mlcommentcontainer} \textcolor{OliveGreen}{#1} \end{mlcommentcontainer}}

  \newcommand{\jncomment}[1]%
  {\begin{jncommentcontainer} \textcolor{blue}{#1} \end{jncommentcontainer}}
}
{ % Turn comments OFF
  \newcommand{\aacomment}[1]{}
  \newcommand{\mlcomment}[1]{}
  \newcommand{\jncomment}[1]{}
}


==> pcrsarlasserreconf.tex <==
\section{Algebraic and semialgebraic proof systems}
\label{sec:algebraic-semialgebraic}

In this section, we show that the size lower bound for resolution in
\refsec{sec:proofs-const-width} 
extends to polynomial calculus
resolution (\PCR) and Sherali-Adams resolution (\SAR)
but not to Lasserre.
%
Due to space constraints,
%    For lack of space 
%    we omit the full proof of the lower bound for \SAR
%    in this extended abstract.
we omit full proofs of the results for \SAR and Lasserre
in this extended abstract.

The main idea 
for the size lower bounds
%    in both cases 
is to  first prove a lower bound on a
parameter analogous to the pigeon-width in
Section~\ref{sec:proofs-const-width},
which 
%    that 
we call
\introduceterm{pigeon-degree} for \PCR and \introduceterm{pigeon-rank}
for \SAR, and then to plug it into the random restriction argument as
in the proof of \reflem{lmm:StrongRestriction}.

\subsection{Refutation 
size
%    length 
lower bound for \PCR}
\label{sec:pcr-length-lower}

Generalizing the terminology in 
\refsec{sec:proofs-const-width}, 
we say that not only
the variables 
$q_{v,w}$ and $z_{v,w}$ of $\TPHP$ 
but also  their twins
$\dualvar{q}_{v,w}$ and $\dualvar{z}_{v,w}$ are said to \emph{mention} pigeon~$v$. 
%    
%    The variables $q_{v,w}$ and $z_{v,w}$ of $\TPHP$ and their twins
%    $\dualvar{q}_{v,w}$ and $\dualvar{z}_{v,w}$ are said to \emph{mention} pigeon~$v$. 
%    
A set of such variables is said to mention a pigeon if some variable in it
does.  The \emph{pigeon-degree} of a monomial is the number of pigeons
that are mentioned by its variables, and the pigeon-degree of a
PCR refutation of $\TPHP$ is the maximum pigeon-degree of any
monomial in the 
% SWITCHING BETWEEN "refutation" and "proof" for the same object in
% the same sentence seems confusing.    
%    proof.
refutation.
% BAD ENGLISH
%    With this terminology, we consider 
We now have
the following analogue of
\reflem{lmm:HardRestrictedFormula}.

\begin{lemma}\label{lmm:pcr-pigeon-degree}
  Every \PCR refutation of $\TPHP$ has pigeon-degree
  at least $\lceil{\frac{k-1}{2}}\rceil$.
\end{lemma}
%
\begin{proof}
%  We show that all \PCR refutations of
%  \eqref{eq:QdefinedRestricted}--\eqref{eq:QinjectiveRestricted} must
%  have a monomial which mentions at least $ \lceil \frac{k-1}{2} \rceil $
%  pigeons.
%  % 
%  In particular we assume to have such a refutation in which all monomials
%  mention at most $M$ pigeons, 
%
We assume we have a \PCR refutation of $\TPHP$ in which all monomials
mention at most $d$~pigeons and transform it into a 
refutation of degree $ d+1 $ of an alternative formulation
$\altPHP$ of the pigeonhole principle from $k$ pigeons to $k-1$
holes described in~\cite{Razborov98LowerBound}.  This formulation does not
have refutations of degree $ \lceil \frac{k-1}{2} \rceil $ or
less~\cite[Theorem~3.9]{IPS99LowerBounds}, from which it follows that
$ d \geq \lceil \frac{k-1}{2} \rceil $.

The alternative formulation $\altPHP$ is defined on variables
$x_{v,w}$ for $v \in [k]$ and $w \in [k-1]$, where $x_{v,w}=1$ means
that pigeon $v$ sits in hole $w$; we stress that this 
interpretation
%      semantic 
of the variables is
the opposite of the one we use 
%    in~$\TPHP$.  
for~$\TPHP$.  
% BAD ENGLISH
%    The polynomials in
%    $\altPHP$ follow, with $ v $ and $ v' $ ranging over $[k]$, and $ w
%    $ and $ w' $ ranging over $ [k-1] $.
Also,
$\altPHP$
is not a (translation of~a) CNF formula but consists of the following
polynomials: 
% Ranges were just specified above; repetition not needed.
%    with $ v $ and $ v' $ ranging over $[k]$, and $ w
%    $ and $ w' $ ranging over $ [k-1] $.
\begin{subequations}
  \begin{align}
    & 
    %          \textstyle 
    1-\sum_{w \in [k-1]}x_{v,w} 
    && \text{for all $ v$,} 
    \label{eq:altPHPdefinedRestrictedA} 
    \\
    & x_{v,w}x_{v',w}
    && \text{for all $ w $ and all $ v\neq v' $,} 
    \label{eq:altPHPdefinedRestrictedB} 
    \\
    & x_{v,w}x_{v,w'}
    && \text{for all $ v $ and all $ w\neq w' $.} 
    \label{eq:altPHPdefinedRestrictedC} 
  \end{align}
\end{subequations} 

To 
obtain
%    get 
a degree-$ (d+1) $ refutation for $ \altPHP $, the first step
is to apply a substitution
$\phpvariableremap$ to the variables in the refutation of
$\TPHP$ in  pigeon-degree~$ d $.
%      pigeon-degree $ d $ for $\TPHP$. 
For $q$\nobreakdash-variables
we
define $\phpvariableremap(q_{v,w}) = 1 - x_{v,w}$ and
$\phpvariableremap(\olnot{q}_{v,w}) = x_{v,w}$, and for
$z$\nobreakdash-variables 
we let
%    define 
$\phpvariableremap(z_{v,w}) = 1 - \sum_{j>w}
x_{v,j}$ and $\phpvariableremap(\olnot{z}_{v,w}) = 1 - \sum_{j \leq
  w} x_{v,j}$.
%
This substitution transforms the refutation of %
the initial formula % DIRTY HACK: saying "the initial formula" here is redundant, but it makes $\TPHP$
% not to overlap to the formula in the previous line
$\TPHP$ into a sequence of polynomials 
over the variables in~$ \altPHP $. 
%    on the variables from $ \altPHP $. 
 
This is not yet a valid refutation, however, and in order to deal with this
we need to show how
%    yet, and to make it so we need to show how
to derive each substituted polynomial in the sequence. 
How to do so
%    This 
depends
on how the polynomial was derived before the substitution.
%
For the inference steps, 
%    Let us focus on the inference steps: 
if we derived $ x p $ from $ p $ then 
$\phpvariableremap(xp)=\phpvariableremap(x)\phpvariableremap(p)$ 
can
be derived from $ \phpvariableremap(p) $ with a sequence of
multiplications and linear combinations, 
and if 
%    ; if 
the polynomial was derived
%    we derived the polynomial
via a linear combination, then the same derivation step is valid for
the substituted polynomials.
%    with a sum inference, then the same sum works after the substitution, too.
%
For the logical axioms of \PCR, the polynomials that result from applying 
$\phpvariableremap$ can be derived from $ \altPHP
$ in constant degree.
% 
The remaining cases are the polynomials obtained applying $
\phpvariableremap $ to the clauses in~\eqref{eq:QdefinedRestrictedA}--\eqref{eq:QdefinedRestrictedC}.
Consider  
$\phpvariableremap(\olnot{z}_{v,w}q_{v,w+1}z_{v,w+1}) $ for $1\leq w < k-3$; the
other cases 
%    of $\phpvariableremap(q_{v,1}z_{v,1})$ and
%    $\phpvariableremap(\olnot{z}_{v,k-3}q_{v,k-2}q_{v,k-1})$ 
are very similar.
We have
% 
\begin{multline}
  \phpvariableremap(\olnot{z}_{v,w}q_{v,w+1}z_{v,w+1}) =\\ 
  \Big(1-\sum_{j \leq w} x_{v,j} \Big) \Big(1-x_{v,w+1} \Big)
  \Big(1-\sum_{j > w+1} x_{v,j} \Big)
\end{multline}
which expands into $1 - \sum_{j \in [k-1]} x_{v,j} + r$
%
%  \begin{multline}
%    \phpvariableremap(\olnot{z}_{v,w}q_{v,w+1}z_{v,w+1}) = 
%    \left(1-\sum_{j \leq w} x_{v,j} \right) 
%    % 
%    \left(1-x_{v,w+1} \right)
%    %
%    \left(1-\sum_{j > w+1} x_{v,j} \right) =\\
%    %
%    1 - \left(\sum_{j \leq w} x_{v,j} \right) - x_{v,w+1} - 
%    \left(\sum_{j > w+1} x_{v,j} \right)  + r
%  \end{multline}
  where $ r $ is a degree-$3$ polynomial on variables $ x_{v,w} $, and
  is in the ideal generated by $ x_{v,w}x_{v,w'} $ and $
  x^{2}_{v,w}-x_{v,w} $.
  % 
  Thus $\phpvariableremap(\olnot{z}_{v,w}q_{v,w+1}z_{v,w+1}) $ can be
  derived from~% 
%      the axioms of 
  $ \altPHP $.
   
  Now we have a refutation of $ \altPHP$. Our substitution 
  exchanges  %%% I assume this is what it meant? --Jakob
%      changes
  variables indexed by pigeon $v$ with degree-$1$ polynomials which
  mention just $v$, 
  and
  therefore each monomial of this refutation mentions at
  most $ d $ pigeons as well.
  %
  We postprocess this refutation by removing all the monomials that
  mention the same pigeon twice or more and all the monomials that mention
  more than one pigeon for the same hole.
  %
  This is possible using the axioms $x_{v,w}x_{v,w'}$ and
  $x_{v,w}x_{v',w}$, and it gives a new refutation of degree at most $
  d+1 $. The lemma follows.
\end{proof}
% \begin{proof}[Proof sketch]
% The proof of the Lemma uses a degree lower bound for a different
% pigeonhole principle formula
% proved in~\cite{IPS99LowerBounds}. In that paper they show that any
% \PCR refutation of their formula requires degree
% $\lceil{\frac{k-1}{2}}\rceil+1$. 
% %
% The core of the proof of the Lemma is that if we have a refutation of
% $ \TPHP $ of pigeon-degree $ d $, we can apply a series of algebraic
% manipulations, substitutions and changes of variables to transform it
% into a degree $ d+1 $ refutation of the formula
% from~\cite{IPS99LowerBounds}. This implies that
% $d \geq \lceil{\frac{k-1}{2}}\rceil$
% \end{proof}


The lower bound on pigeon-degree in Lemma~\ref{lmm:pcr-pigeon-degree}
together with Lemma~\ref{lmm:StrongRestriction} imply the size lower
bound for \PCR.

\begin{theorem}
  Let $k = k(n)$ be any integer-valued function such that $k(n) \leq
  n/4\log n$. Any \PCR refutation of $ \erphpknk $ has size
  $\Omega \bigl( {n^{\lceil(k-1)/2\rceil}/(3k^2\log n)^{k}} \bigr) $.
\end{theorem}
\begin{proof}
  Let $\monoset{M}$ be the set of monomials appearing in a \PCR refutation of
  $\erphpknk$.
  %
  We hit the refutation with a random restriction
  $ \rstd $ distributed according to $ \PADistribution $. 
  Since restrictions preserve 
%      soundness of  \PCR inferences
  \PCR derivations
  we obtain a
  refutation of $ \restrict{\erphpknk}{\rstd} $, which as before is \TPHP.

  Assume that $ \cardinality{\monoset{M}} <
  {{n^{\lceil(k-1)/2\rceil}}/{(3k^{2}\log n)}^{k}}$.
  % WHY IS THE COMMENT BELOW NEEDED? LEMMA 4 ALREADY EXPLICITLY COVERS TERMS/MONOMIALS.
%      , and observe that
%      the monomials in $\monoset{M}$ 
%      % are essentially 
%      behave as disjunctions of
%      variables.
  %
%      By \reflem{lmm:StrongRestriction} with $\ell = \left\lceil
%        \frac{k-1}{2}\right\rceil$ and union bound over the size of $ \monoset{M}$,
  Applying
  \reflem{lmm:StrongRestriction} with 
  $\ell = \left\lceil \frac{k-1}{2}\right\rceil$ 
  and taking a union bound over 
  the monomials in~%
%      the size of 
  $ \monoset{M}$,
  we conclude that
  there must be at least one restriction $ \rstd $ in the support of
  $\PADistribution $ such that the pigeon-degree of
  $\restrict{\proofstd}{\rstd}$ is at most $\left\lceil \frac{k-1}{2}
  \right\rceil -1$
%    , assuming $ n $ large enough.
  if $ n $ is large enough.
  % BAD ENGLISH
%      This contradicts Lemma~\ref{lmm:pcr-pigeon-degree}, thus
%      $\cardinality{\monoset{M}}$ 
%      must be at least 
%      $ {{n^{\lceil(k-1)/2\rceil}}/{(3k^{2} \log n)}^{k}} $.
  This contradicts \reflem{lmm:pcr-pigeon-degree}, and hence
  $\cardinality{\monoset{M}}$ 
  must be at least 
  $ {{n^{\lceil(k-1)/2\rceil}}/{(3k^{2} \log n)}^{k}} $.
\end{proof}


\subsection{Refutation length lower bound for \SAR}

The definition of pigeon-rank is the analogue of pigeon-width for
resolution (see Section~\ref{sec:proof-lower-bound}) and pigeon-degree
for \PCR (see Section~\ref{sec:pcr-length-lower}). 
%
The \emph{pigeon-rank} of an \SAR
refutation of $\TPHP$ is
the maximum pigeon-degree among 
% WHAT?!
%    the one of polynomials
the polynomials
$\prod_{i \in \pLit_t} x_i \cdot \prod_{i \in \nLit_t} (1-x_i) \cdot
\polyp_t$ in Equation~\eqref{eqn:SAdefinition}.

% WE ARE NOT STATING NAMES FOR OTHER PAPERS IN THIS SECTION...
%    Dantchev, Martin and Rhodes~\cite{DantchevMartinRhodes2009Tight} 
%    proved a rank lower bound on
%    \SAR refutations of $\PHPk$. 
In~\cite{DantchevMartinRhodes2009Tight}, 
a rank lower bound was proven on \SAR refutations of $\PHPk$. 
We extend this to a pigeon-rank lower bound for~$\TPHP$.
%    Here we extend it to $\TPHP$ and to pigeon-rank. 
%
The proof is omitted in this extended abstract: the intuition is that
a set of inequalities does not admit a refutation of pigeon-rank $ r $
if there is a family of distributions on partial assignments as follows.
\begin{enumerate}\itemsep=0pt
  \item There is a distribution for every set of variables that
  mentions at most $ r $ pigeons;
  \item the distributions of two sets of variables are consistent on
  their intersection;
  \item no initial inequality or logical axiom is falsified by any
  assignment in the support of any distribution.
\end{enumerate} 
%
Thus the proof of the following lemma (omitted here) amounts to showing
that such a family of distributions exists for $ r=k-1 $.

\begin{lemma}\label{lmm:sar-pigeon-rank}
  Every \SAR refutation of $\TPHP$ has pigeon-rank at least $k$.
\end{lemma}

The lower bound on pigeon-rank in Lemma~\ref{lmm:sar-pigeon-rank}
together with Lemma~\ref{lmm:StrongRestriction} imply the size lower
bound for \SAR.

\begin{theorem}
  Let $k = k(n)$ be any integer-valued function such that $k(n) \leq
  n/4\log n$. Any \SAR refutation of $ \erphpknk $ has size
  $\Omega \bigl( {n^k/(3k^2\log n)^{k}} \bigr) $.
\end{theorem}

\begin{proof}
  % % 
  % Consider a \SAR refutation of $\erphpknk$ and let be $ M$ the
  % set of monomial appearing in such refutation.
  % 
  Let $\monoset{M}$ be the set of monomials appearing in a \SAR refutation of
  $\erphpknk$.
  %
  We hit the refutation with a random restriction
  $ \rstd $ distributed according to $ \PADistribution $.  
  Since restrictions preserve soundness of \SAR proofs
  we obtain a
  refutation of $ \restrict{\erphpknk}{\rstd} $, which is \TPHP.

% VARYING THE PROSE EVER SO SLIGHTLY...
Suppose now that
%      Assume that 
  $ \cardinality{\monoset{M}} < n^{k}/{(3k^{2} \log n)}^{k}$.
% AGAIN, LEMMA 4 WORKS PERFECTLY FINE WITHOUT THE FOLLOWING PHRASE
%    , and
%      observe that the monomials in $\monoset{M}$ 
%      % are essentially to
%      behave as
%      conjunctions of variables. 
% WE TAKE THE UNION BOUND OVER THE SET, NOT OVER THE SIZE OF THE SET, RIGHT?
%      By \reflem{lmm:StrongRestriction} with $\ell = k$ and union bound over
%      the size of $\monoset{M}$, 
  Using \reflem{lmm:StrongRestriction} with $\ell = k$ and a union
  bound argument for~$\monoset{M}$, 
  we conclude that
  there 
  exists
%      must be 
  at least one restriction $ \rstd $
  in the support of $\PADistribution $ such that the pigeon-rank of
  $\restrict{\proofstd}{\rstd}$ is at most $k-1$, 
  assuming 
  that
  $ n $ large enough.
  %
  But
  this contradicts \reflem{lmm:sar-pigeon-rank},
  and hence the theorem follows.
% BAD ENGLISH
%      , thus
%      $\cardinality{\monoset{M}}$ must be at least $ n^{k}/{(3k^{2} \log n)}^{k} $.
  % ,
  % which is $ n^{\Omega(k)} $ when $ k=O(n^{c}) $ and $ c<1/2 $.
  % %
  % If $k$ is further restricted to $\Littleoh{(\log n) / (\log \log
  %   n)^{2}}$, then $ \cardinality{M} > n^{k-o(1)} $.
\end{proof}

\subsection{Upper bound for Lasserre proofs}
\label{sec:upper-bound-lasserre}
\label{sec:lasserre}

Our lower bound does not extend all the way up to Lasserre
refutations. 
% WHY "indeed"?
%    Indeed 
In the full version of this paper we show that
$\rphpknk$ and $\erphpknk$ have Lasserre refutations of size
polynomial in $ k $ and $ n $.
More specifically,
% WHY "in particular"?
%    In particular 
we show that $\rphpknk$ and $\erphpknk$ have
constant-rank Lasserre refutations, for a constant that is independent
of $k$ and $n$, 
%    and that implies immediately the upper bound on
%    refutation size.
and this immediately implies the upper bound on
refutation size.
Let us state the concrete lemma for reference.

\begin{lemma}
  $\rphpknk$ and $\erphpknk$ have Lasserre
  refutations of rank $9$.
\end{lemma}

The proof builds on Lemma~1.5 in~\cite{LovaszSchrijver1991Cones} which
can be used to 
construct
%    get 
a rank-$2$ Lasserre refutation of the 
(standard) pigeonhole principle formula
$\PHP^k_{k-1}$. A similar proof for $\PHP^k_{k-1}$ also
appears in~\cite{GrigorievHirschPasechnik2002Complexity}.





==> semialgebraic.tex <==
\section{Semi-algebraic proofs}

\subsection{Definitions}

For this section all polynomials have real coefficients and formal
variables within $x_1,\ldots,x_n$. A polynomial inequality is a formal
expression $P \geq 0$ where $P$ is a polynomial written as the sum of
its non-zero monomials. The following inference rules are called
\emph{positive linear combination}, \emph{multiplication} and
\emph{positivity of squares}:
\begin{equation}
\frac{P \geq 0 \;\;\;\;\;\;\;\;\; Q \geq 0}{\lambda P + \mu Q \geq 0}
\;\;\;\;\;\;\;\;\;\;\;\;\; 
\frac{P \geq 0 \;\;\;\;\;\;\;\;\; Q \geq 0}{PQ \geq 0}
\;\;\;\;\;\;\;\;\;\;\;\;\; 
\frac{}{P^2 \geq 0}
\label{eqn:semialgebraicrules}
\end{equation}
where $P$ and $Q$ are polynomials and $\lambda, \mu \geq 0$ are
non-negative reals. These inference rules are sound over the reals: if
the hypotheses are satisfied by some $\vectorx \in \reals^n$, then the
conclusion is also satisfied by the same $\vectorx$. In applications
to combinatorial problems where the variables are supposed to take
values in $\{0,1\}$, the following \emph{variable-axioms} are also
considered:
\begin{equation}
\frac{}{x \geq 0}
\;\;\;\;\;\;\;\;\;
\frac{}{1-x \geq 0}
\;\;\;\;\;\;\;\;\;
\frac{}{x - x^2 \geq 0}
\;\;\;\;\;\;\;\;\;
\frac{}{x^2 - x \geq 0}
\label{eqn:variableaxioms}
\end{equation}
where $x$ is a variable. 

Let $S$ be a set of polynomial inequalities. A \emph{semialgebraic
  proof} from $S$ is a sequence of polynomial inequalities, each of
which belongs to $S$ or is one of the trivial inequalities $1 \geq 0$
and $0 \geq 0$, or is obtained from previous inequalities in the
sequence by positive linear combinations, multiplications, or
positivity of squares. The \emph{length} of the proof is the number of
polynomial inequalities in the sequence, the \emph{size} is the total
number of monomials that appear in the proof, and the \emph{degree} is
the maximum degree of the polynomials that appear in the proof. A
\emph{refutation} is a proof of the trivially unsatisfiable polynomial
inequality $-1 \geq 0$. In the \emph{semidefinite Lov\'asz-Schrijver}
proof system $\LSPLUS$ the axiom-variables are also allowed, but the
four rules in \eqref{eqn:semialgebraicrules} are restricted to the
following forms:
\begin{equation}
\frac{P \geq 0 \;\;\;\;\;\; Q \geq 0}
{\lambda P + \mu Q \geq 0}
\;\;\;\;\;\;\;\;\;\; 
\frac{P \geq 0}{x P \geq 0}
\;\;\;\;\;\;\;\;\;\; 
\frac{P \geq 0}{(1-x) P \geq 0}
\;\;\;\;\;\;\;\;\;\; 
\frac{}{P^2 \geq 0}
\label{eqn:lovaszschrijver}
\end{equation}
where $x$ is a variable, and $P$ is such that the conclusion in the
rule is a \emph{quadratic} polynomial, i.e. its formal degree is at
most two. The \emph{degree-$k$ semidefinite Lov\'asz-Schrijver} proof
system $\LSPLUS(k)$ is defined similarly except that the polynomial
$P$ in \eqref{eqn:lovaszschrijver} is such that the conclusion in the
rule has degree at most $k$. Thus $\LSPLUS = \LSPLUS(2)$.  A
\emph{Lasserre proof of rank $k$} is an $\LSPLUS(k)$-proof of special
form: all applications of positive linear combinations come after all
applications of multiplications, positivity of squares, and axioms.
The \emph{linear programming} version $\LS(k)$ of $\LSPLUS(k)$ is the
restriction in which positivity of squares is not allowed. A
\emph{Sherali-Adams (SA) proof of rank $k$} is an $\LS(k)$-proof of
special form: all applications of positive linear combinations come
after all applications of multiplications and axioms.

Finally we introduce versions of all these proof systems in which each
variable $x$ has a formal copy $x'$ and the \emph{complementarity
  axioms} enforce the identity $x' = 1-x$:
\begin{equation}
\frac{}{x + x' - 1 \geq 0}
\;\;\;\;\;\;\;\;\;\; 
\frac{}{1 - x - x' \geq 0}
\label{eqn:complementarity}
\end{equation}
These variants are useful to avoid the combinatorial explosion in the
number of monomials that occur in expressions such as $\prod_{i \in I}
(1-x_i)$. As a polynomial in the variables $x_1,\ldots,x_n$ this
polynomial has $2^{|I|}$ monomials, but in the presence of
\eqref{eqn:complementarity}, this can be written equivalently as a
single monomial $\prod_{i \in I} x'_i$.  We write $\LSPLUSR(k)$, read
degree-$k$ semi-definite Lov\'asz-Schrijver Resolution, for the
extension of $\LSPLUS(k)$ by \eqref{eqn:complementarity}, and
similarly for $\LS(k)$. Lasserre Resolution proofs of rank $k$ and SA
Resolution proofs of rank $k$ are defined accordingly.

\subsection{Elementary facts}

To every pair of sets of variables $Y, Z \subseteq \{x_1,\ldots,x_n\}$
we associate polynomials $M(Y,Z) := \prod_{x \in Y} (1-x) \prod_{x \in
  Z} x$ and $S(Y,Z) := \sum_{x \in Y} x + \sum_{x \in Z} (1-x)$, with
$M(\emptyset,\emptyset) = 1$ and $S(\emptyset,\emptyset) = 0$.  Note
that $M(Y,Z)$ has degree $|Y|+|Z|$, and $S(Y,Z)$ and is a linear
polynomial. The polynomials $M'(Y,Z)$ and $S'(Y,Z)$ are defined
similarly except that every term of the form $(1-x)$ is replaced by
the copy $x'$ of the variable $x$.

In the presence of the variable-axioms \eqref{eqn:variableaxioms}, a
clause $C$ of the form $\Lor_{x \in Y} x \vee \Lor_{x \in Z}
\olnot{x}$ will be represented as a polynomial inequality in four
different ways: the $M$-representation is the polynomial inequality
$-M(Y,Z) \geq 0$, the $M'$-representation is the inequality $-M'(Y,Z)
\geq 0$, the $S$-representation is the inequality $S(Y,Z)-1 \geq 0$,
and the $S'$-representation is the inequality $S'(Y,Z)-1 \geq 0$. We
write $M(C)$, $M'(C)$, $S(C)$ and $S'(C)$ for these
representations. Observe that if $C$ is the empty clause, then all
these representations give the trivially unsatisfiable inequality $-1
\geq 0$. For a CNF formula $F$ we write $M(F)$ for the set of
polynomial inequalities that results from applying the $M$-operator
to each clause. The notation  $M'(F)$, $S(F)$ and
$S'(F)$ is readily explained.

The following easy lemmas are surely well-known; we provide a proof
for completeness.

\begin{lemma} \label{lem:convert}
  Let $C$ be a $k$-clause. The following hold:
  \begin{enumerate} \itemsep=0pt
  \item $M(C)$ has an SA-proof of rank $k$ and size $O(k
    2^k)$ from $S(C)$,
  \item $M'(C)$ has an SAR-proof of rank $k$ and
    size $O(k^2)$ from $S'(C)$.
  \end{enumerate}
\end{lemma}

\begin{proof}
  Let us prove \emph{1.} first. If $C$ is the empty clause then the
  claim is obvious since in that case $M(C) = S(C)$. Assume then that
  $C$ is not empty. Pick an arbitrary literal $\ell$ in $C$ so that
  $C$ has the form $\ell \lor C'$ with $C'=\Lor_{x \in Y} x \vee
  \Lor_{x \in Z} \olnot{x}$ and $ |Y|+|Z|<k $. Let $v$ be the variable
  of the literal $\ell$. Inequality $ S(C) $ has the form $ t +
  S(Y,Z) - 1 \geq 0 $, where $ t=v $ if $ \ell $ is positive and
  $ t = 1 - v $ otherwise.

  Repeatedly multiplying $S(C)$ by each $(1-x)$ for $x \in Y$ and each
  $x$ for $x \in Z$ gives a polynomial inequality of degree at most
  $k$ of the form
  \begin{equation}
    t M(Y,Z)
    +
    \sum_{x \in Y} x M(Y,Z)
    + 
    \sum_{x \in Z} (1-x) M(Y,Z)
    -
    M(Y,Z) \geq 0. \label{eqn:almost}
  \end{equation}
  Note that, for $i \in \{1,\ldots,|Y|+|Z|\}$, the $i$-th polynomial
  inequality in this process has $O(2^i)$ monomials, for a total of
  $O(2^k)$ monomials. For each $x \in Y$, repeatedly multiplying the
  axiom $x^2 - x \geq 0$ by each $(1-y)$ for $y \in Y \setminus \{x\}$
  and by each $ y $ for $y \in Z$ gives the polynomial inequality $-x
  M(Y,Z) \geq 0$.  For each $x \in Z$, repeatedly multiplying the
  axiom $x^2 - x \geq 0$ by each $y$ for $y \in Z \setminus \{x\}$ and
  by each $1-y$ for $y \in Y$ gives the polynomial inequality
  $-(1-x)M(Y,Z) \geq 0$.  These are at most $k$ polynomial
  inequalities and each produced no more than $O(2^k)$ monomials in
  the process of their proof.  Adding up all the derived inequalities
  gives $-(1-t)M(Y,Z) \geq 0$, which is exactly $M(C)$,
  producing no more than $O(k 2^k)$ monomials in total.  The degree of
  all these polynomials does not exceed $k$ and all applications of
  positive linear combinations come after all other rule
  applications. Thus, the proof is an SA-proof of rank $k$ and size
  $O(k 2^k)$.

  For \emph{2.} the proof is the same replacing each $(1-x)$ by $x'$
  and $M(Y,Z)$ by $M'(Y,Z)$. Now $ t =v' $ if $ \ell $ is a
  negative literal.  In the end we get $ -(1-t)M'(Y,Z)\geq 0
  $. If $t=1-v$ we are done, otherwise we add
  $(1-v-v')M(Y,Z)\geq 0$ which has a derivation from axiom
  (\ref{eqn:complementarity}) of rank $ k$ and size $O(k^{2})$.  For
  the size-bound, the proof of \eqref{eqn:almost} involves $O(k^2)$
  monomials, and this dominates the total size.
\end{proof}

The point of converting the $S$-representation of a clause into its
$M$-representation is that the inequality
\begin{equation}
M(A \vee x) + M(B \vee \olnot{x}) - M(A \vee B) \geq 0
\label{eq:resolutioninM}
\end{equation} 
has an efficient SA-proof and hence the resolution rule can simulated
by addition.  Getting~\eqref{eq:resolutioninM} requires a little
argument, so we state it as a lemma.

\begin{lemma} \label{lem:simulate}
Let $x$ be a variable, let $A$ and $B$ be clauses in which $x$ does
not appear, and let $k$ be the width of $A \vee B$.  The following
hold:
\begin{enumerate} \itemsep=0pt
\item $M(A \vee x) + M(B \vee \olnot{x}) -
M(A \vee B) \geq 0$ has an SA proof of rank $k+1$ and size $O(k2^{k})$,
\item $M'(A \vee x) + M'(B \vee \olnot{x}) - M'(A \vee B) \geq 0$ has
  an SAR proof of rank $k+1$ and size $O(k^2)$.
\end{enumerate}
\end{lemma}

\begin{proof}
We prove \emph{1.} since \emph{2.} is even easier.  To prove \emph{1.}
it suffices to get the inequalities $M(A \vee x) - M(A \vee B \vee x)
\geq 0$ and $M(B \vee \olnot{x}) - M(A \vee B \vee \olnot{x}) \geq 0$
since one addition will give the result by using the identity
$$
M(A \vee B \vee x) + M(A \vee B \vee \olnot{x}) = M(A \vee B).
$$

For this, it suffices to show how
to get $M(Y,Z) - M(Y \cup Y', Z \cup Z') \geq 0$ for any four sets
$Y$, $Y'$, $Z$ and $Z'$. Let $Y' = \{ y_1,\ldots,y_t\}$ and $Z' = \{
z_1,\ldots,z_s\}$, and define $Y_i = Y \cup \{ y_1,\ldots,y_i \}$ and
$Z_j = Z \cup \{ z_1,\ldots,z_j \}$ for $i \in \{0,\ldots,t\}$ and $j
\in \{0,\ldots,s\}$, respectively. First note that, for any sets of
variables $Y''$ and $Z''$, the inequality $M(Y'',Z'') \geq 0$ can be
obtained by starting at the trivial inequality $1 \geq 0$, multiplying
it by $x$ for all $x$ in $Y''$, and then multiplying the result by
$1-x$ for all $x$ in $Z''$. Second note that, for $i \in
\{1,\ldots,t\}$, the inequality $M(Y_{i-1},Z) - M(Y_i,Z) \geq 0$ can
be obtained by starting at $M(Y_{i-1},Z) \geq 0$ and multiplying it by
$1-y_i$. Third note that, for $j \in \{1,\ldots,s\}$, the inequality
$M(Y_t,Z_{j-1}) - M(Y_t,Z_j) \geq 0$ can be obtained by starting at
$M(Y_t,Z_{j-1}) \geq 0$ and multiplying it by $z_j$. Now, adding all
the derived inequalities together we get a telescoping sum that
simplifies to $M(Y_0,Z_0) - M(Y_s,Z_t) \geq 0$.  This is precisely
$M(Y,Z) - M(Y \cup Y',Z \cup Z') \geq 0$.

To estimate the rank and size, observe that all derived inequalities
have degree at most $k+1$ and size at most $O(2^k)$, for a total size
of $O(k2^k)$.
\end{proof}

Next we use this lemma to simulate resolution.

\begin{lemma}
  Let $F$ be a CNF formula.  If $F$ has a resolution refutation of
  width $k$ and size $s$, then $S(F)$ has an SA-refutation of rank
  $k+1$ and size $O(k2^k s)$, and an SAR-refutation of rank $k+1$ and
  size $O(k^2 s)$.
\end{lemma}

\begin{proof}
  Both statements have the same proof using the corresponding part of
  Lemmas~\ref{lem:convert} and~\ref{lem:simulate}. We outline the
  proof of the first statement only. For each clause $C$ in $F$,
  derive $M(C)$ from $S(C)$ using Lemma~\ref{lem:convert}.  Next, for
  each resolution step deriving $A \vee B$ from two clauses $A \vee x$
  and $B \vee \olnot{x}$ in $F$, derive the inequality $M(A \vee x) +
  M(B \vee \olnot{x}) - M(A \vee B) \geq 0$ using
  Lemma~\ref{lem:simulate}. In order to get the refutation we are
  going to combine all these inequalities by a big positive linear
  combination with appropriate weights that we define next.

  Consider the DAG of the resolution refutation with edges oriented
  from the initial clauses towards the empty clause. We assign a
  weight $w(C)$ to each clause $C$ in this DAG by traversing it as
  follows: the empty clause gets weight $1$, and if all successors of
  a clause have already been assigned weights, then the clause gets
  the sum of the weights of its successors as weight for itself.  Once
  weights are assigned, we take the positive linear combination of all
  derived inequalities using $w(C)$ as multiplier for the inequality
  corresponding to the inference that produced $C$. What we get is a
  proof of $-w(0) M(0) \geq 0$. Since $M(0) = 1$ and the empty clause
  has weight $1$, this is a refutation of $S(F)$. By
  Lemmas~\ref{lem:convert} and~\ref{lem:simulate}, each derived
  inequality is derived by an SA-proof of rank $k+1$ and size
  $O(k2^k)$. The rest of inferences are just positive linear
  combinations. The result is an SA refutation of rank $k+1$ and size
  $O(k2^k)$.
\end{proof}

Next we show that semialgebraic proofs do not become more complex
under restrictions.  If $P$ is a polynomial and $\rho$ is a partial
assignment, we write $\restrict{P}{\rho}$ for the restriction of $P$
by $\rho$, i.e. the polynomial that results from replacing each
variable $x$ in $\dom(\rho)$ by $\rho(x)$ and its copy $x'$ (if it
exists) by $1-\rho(x)$.  If $S$ is a set of polynomial inequalities,
we write $\restrict{S}{\rho}$ for the set of polynomial inequalities
that results from restricting each polynomial in these inequalities to
$\rho$.

\begin{lemma}
  For every set of polynomial inequalities $S$, every polynomial $P$
  and every partial assignment $\rho$, if $P$ has an SA-proof of rank
  $k$ and size $s$ from $S$, then $\restrict{P}{\rho}$ has an SA-proof
  of rank $k$ and size at most $s$ from $\restrict{S}{\rho}$. The same
  holds for SAR with respect to the $S'$-representation.
\end{lemma}

\begin{proof}
  This is an easy induction on the length of the proof. To see this,
  first observe that variable-axioms either stay unchanged by the
  restriction or become one of the trivial inequalities $1 \geq 0$ or
  $0 \geq 0$.  Similarly, the literal multiplication rules either
  apply as they are to the restricted polynomial, or become a trivial
  derivation of $\restrict{P}{\rho} \geq 0$ from $\restrict{P}{\rho}
  \geq 0$ itself, or become a trivial inequality of the form $0 \geq
  0$. Finally, the complementarity axioms $x + x' - 1 \geq 0$ and $1 -
  x - x' \geq 0$ either stay unchanged, or become the trivial
  inequality $0 \geq 0$.  The rest of rules apply as they are.
\end{proof}

% Finally we show that rank in Sherali-Adams and Sherali-Adams Resolution
% concide.
% 
% \begin{lemma} \label{lem:SAvsSAR}
% Let $S'$ be a set of polynomial inequalities on
% the variables $x_1,\ldots,x_n,x'_1,\ldots,x'_n$ and let $S$ be the
% result of replacing each $x'_i$ by $1-x_i$ in $S'$. The following are
% equivalent:
% \begin{enumerate} \itemsep=0pt
% \item $S$ has a Sherali-Adams refutation of rank $k$,
% \item $S'$ has a Sherali-Adams Resolution refutation of rank $k$.
% \end{enumerate}
% \end{lemma}
% 
% \begin{proof}
% In the direction from 2. to 1. just replace each occurrence of a
% variable $x'_i$ in the proof by $1-x_i$ and observe that the
% complementarity axioms $x'_i + x_i - 1 \geq 0$ and $1 - x_i - x'_i
% \geq 0$ become the trivial inequality $0 \geq 0$ and all the other
% rules remain valid. The direction from 1. to 2. is left to the reader
% (it is not used below anyway)\footnote{\aacomment{Any objection to
%     this? It should be analogous to the corresponding result on degree
%     in PC vs PCR.}}.
% \end{proof}

\subsection{Lower bounds on Sherali-Adams (mentioning-)rank}

For our application we need to prove lower bounds on a more general
notion of rank in which we count, not the degree, but the maximum
number of occurrences of variables in a monomial, up to a given
equivalence relation on the variables. We introduce this concept
first.

Let $V$ be a set of variables partitioned into $p$ non-empty blocks
$V_1,\ldots,V_p$. For a set of variables $X$ and a block-number $i \in
\{1,\ldots,p\}$, we say that $X$ mentions block $i$ if it contains
some variable in $V_i$. We say that a polynomial mentions block $i$ if
its set of variables mentions block $i$, and that a polynomial
inequality mentions $i$ if its polynomial does.  For $k \in
\{1,\ldots,p\}$, let $W^k(V_1,\ldots,V_p)$ denote the collection of
all subsets of variables in $V$ that mention at most $k$ blocks. If
the blocks are clear from the context we write just $W^k$. An SA-proof
of \emph{mentioning-rank} $k$ is one in which all its monomials
mention at most $k$ blocks. For SAR mentioning-rank is defined
similarly with the convention that the copy $x'$ of a variable $x$
belongs to the same block as $x$.

Let $k \geq 0$ be an integer and let $S$ be a set of polynomial
inequalities on the variables $V$.  A $k$-\emph{block consistent
  family of distributions} for $S$ is a collection of probability
distributions $\Pi_X$ over assignments $\{0,1\}^X$, as $X$ ranges over
$W^k$, that satisfies the following properties:
\begin{enumerate} \itemsep=0pt
\item for every $X$ in $W^k$ and every polynomial inequality $P \geq
  0$ in $S$ that has all its variables in $X$, every assignment in the
  support of $\Pi_X$ satisfies $P \geq 0$,
\item for every $X$ and $Y$ in $W^k$ such that $X \subseteq Y$ and
  every $f \in \{0,1\}^X$ we have $\Pi_X(f) = \sum_{g \supseteq f}
  \Pi_Y(g)$ for $g$ ranging over $\{0,1\}^Y$.
\end{enumerate}
If such a family of distributions exists we say that $S$
admits a $k$-block consistent family of distributions. 

\begin{lemma} \label{lem:sufficient}
  Let $k \geq 1$ be an integer and let $S$ be a set of polynomial
  inequalities all whose polynomials mention at most $k$ blocks. If
  $S$ has an SA-refutation of mentioning-rank $k$, then $S$ does not
  admit a $k$-block consistent family of distributions.
\end{lemma}

\begin{proof}
  Think of each $W^k$ as a new formal variable. For each monomial $M$,
  let $X_M$ denote the set of variables in $M$ and let $a_M$ denote
  the coefficient of $M$. For every polynomial $P$ all whose monomials
  mention at most $k$ blocks, let $\hat{P}$ be the linear form on the
  variables $W^k$ that is obtained from $P$ by replacing each monomial
  $M$ by $a_M X_M$. Note that $\hat{P}$ can also be thought of as a
  multilinear polynomial on the original variables.  For a set of
  variables $Y$, let $1_Y$ denote the assignment $\{ x \mapsto 1 : x
  \in Y \}$, and for a monomial $M$, let $1_M = 1_{X_M}$.

  Let $P_1,\ldots,P_m,P_{m+1},\ldots,P_t$ be the polynomials in an
  SA-refutation of mentioning-rank $k$ from $S$, where $P_m \geq 0$ is
  the last inequality in the phase in which positive linear
  combinations are not used.  Assuming for contradiction that
  $\{\Pi_X\}$ is a $k$-block consistent family for $S$, we will show
  that the real assignment $a : W^k \rightarrow \reals$ defined by
  \[
  a(X) = \Pi_X(1_X)
  \] 
  satisfies $a(\hat{P}_i) \geq 0$ for every $i \in
  \{1,\ldots,m\}$. Since every $\hat{P}_i$ with $i \in
  \{m+1,\ldots,t\}$ is a positive linear combination of the
  $\hat{P}_\ell$'s with $\ell \in \{1,\ldots,m\}$, this will show that
  $a(\hat{P}_i) \geq 0$ for every $i \in \{m+1,\ldots,t\}$ and
  contradict the fact that $P_t = -1$ and hence $\hat{P}_t = -1$.

  Let us check that $a$ satisfies every $\hat{P}_i \geq 0$ with $i \in
  \{1,\ldots,m\}$. We prove a stronger claim: if $X_i$ is the set of
  variables in $P_i$ and $\Exp_{X_i}$ denotes expectation under the
  distribution $\Pi_{X_i}$, then $a(\hat{P}_i) = \Exp_{X_i}(P_i)$ and
  every assignment in the support of $\Pi_{X_i}$ satisfies the
  inequality $P_i \geq 0$.  For the first condition, the one stating
  that $a(\hat{P}_i) = \Exp_{X_i}(P_i)$, it suffices to proceed for
  each monomial $M$ in $P$ separately:
  \begin{align*}
  a(\hat{M}) & = c_M a(X_M) = c_M \Pi_{X_M}(1_{M}) = c_M \sum_{g \supseteq
    1_{M}} \Pi_{X_i}(g) = \Exp_{X_i}(M).
  \end{align*}
  The third follows from property 2. in the definition of $k$-block
  consistent family and the forth follows from the fact that on every
  assignment in $\{0,1\}^{X_i}$ a monomial with all its variables in
  $X_i$ takes the same value as its multilinear version (since $x^2 =
  x$ on $\{0,1\}$). Adding over all monomials we get $a(\hat{P}_i) =
  \Exp_{X_i}(P_i)$. For the second condition, the one stating 
  that every assignment in the support of $\Pi_{X_i}$ satisfies 
  the inequality $P_i \geq 0$, we proceed by induction on $i$.
  
  If $P_i \geq 0$ is a variable-axiom, the claim is obvious since
  every assignment in the support of $\Pi_{X_i}$ gives value $0$ or
  $1$ to the variable. If $P_i = P$ for some inequality $P \geq 0$ in
  $S$, the claim is precisely property 1. in the definition of
  $k$-block consistent family. It remains to check the case that $P_i
  \geq 0$ is derived from some previous $P_j \geq 0$ with $1 \leq j
  \leq i-1$ by multiplication. Both cases $P_i = x P_j$ and $P_i =
  (1-x) P_j$ have similar proofs, so let us consider the first.  If
  $x$ does not appear in $P_i$ then $P_j=P_i=0$ and the claim is
  obvious. Suppose then that $x$ appears in $P_i$.  For each
  assignment $f$ in the support of $\Pi_{X_i}$ we have either $f(x) =
  0$ or $f(x) = 1$. In the first case, the inequality $xP_j \geq 0$ is
  obviously satisfied. In the second case, the inequality $xP_j \geq
  0$ reduces to $P_j \geq 0$. If $x$ appears in $P_j$, then $X_j =
  X_i$ and $f$ satisfies $P_j \geq 0$ by induction hypothesis. If $x$
  does not appear in $P_j$, let $g$ be the restriction of $f$ to $X_j$
  and observe that, by property 2.  in the definition of $k$-block
  consistent family, $g$ is in the support of $\Pi_{X_j}$. By
  induction hypothesis $g$ satisfies $P_j \geq 0$. Since $f \supseteq
  g$ and the variables in $\dom(f) \setminus \dom(g)$ do not appear in
  $P_j$, also $f$ satisfies $P_j \geq 0$, and hence $P_i \geq 0$. This
  concludes the induction and the proof of the lemma.
\end{proof}

We apply the preceding lemma to prove mentioning-rank lower bounds for
the pigeonhole principle. Let $\PHP^k_{k-1}$ denote the clauses for
the pigeonhole principle and let $3\PHP^k_{k-1}$ be its 3-CNF-ed
version; in other words, the clauses
\eqref{eq:QdefinedRestricted}--\eqref{eq:QinjectiveRestricted} for $S
= [k]$.  Dantchev, Martin and Rhodes
\cite{DantchevMartinRhodes2009Tight} proved a rank lower bound on
SA-refutations of $\PHP^k_{k-1}$. Here we extend it to $3\PHP^k_{k-1}$
and to mentioning-rank with the partition of the variables into blocks
according to the (unique) pigeon that they mention. For this
particular choice of the partition, we rename mentioning-rank into
\emph{pigeon-rank}:

\begin{theorem}\label{thm:SAPigeonRankLowerbound}
  For every $k \geq 2$, the system of inequalities $S(3\PHP^k_{k-1})$
  does not have SAR-refutations of pigeon-rank $k-1$.
\end{theorem}

\begin{proof}
  First note that by replacing each variable $x'$ by $1-x$ we
  transform an SAR-proof into an SA-proof of the same
  pigeon-rank. Thus, by Lemma~\ref{lem:sufficient} it will suffice to
  build a $(k-1)$-block consistent family of distributions for
  $S(3\PHP^k_{k-1})$. Observe that each polynomial inequality in this
  formula mentions at most two pigeons.  For every set $X$ of
  variables than mention up to $k-1$ pigeons, the distribution $\Pi_X$
  is defined as follows:
  \begin{enumerate} \itemsep=0pt
  \item let $A$ be the set of at most $k-1$ pigeons that are mentioned
    by the variables in $X$,
  \item let $m$ be a uniformly chosen one-to-one map $m : A \rightarrow [k-1]$,
  \item for every $q_{v,w}$-variable in $X$, set it to $1$ if
    $m(v) = w$ and set it to $0$ otherwise,
  \item for every $z_{v,w}$-variable in $X$, set it to $1$ if
    $m(v) > w$ and set it to $0$ otherwise.
  \end{enumerate}
  Let us check conditions 1. and 2.. For 1., fix a set $X$ that
  mentions up to $k-1$ pigeons, let $C$ be a clause in
  $\PHP^{k}_{k-1}$ that has all its variables in $X$, and let $f \in
  \{0,1\}^X$ be an assignment in the support of $\Pi_X$. Let $A$ be
  the set of at most $k-1$ pigeons that are mentioned in $X$ and let
  $m$ be any one-to-one map $m : A \rightarrow [k-1]$ that witnesses
  that $f$ is in the support of $\Pi_X$. If $C$ is a clause of type
  \eqref{eq:QdefinedRestricted} for some pigeon $v \in [k]$, then $v$
  belongs to $A$ and $C$ is satisfied by the assignment $f$ by
  construction. If $C$ is a clause of type
  \eqref{eq:QinjectiveRestricted} for two pigeons $v,v' \in [k]$ with
  $v \not= v'$ and a hole $w \in [k-1]$, then again $v$ and $v'$
  belong to $A$ and $C$ is satisfied by the assignment $f$ by
  construction.

  For 2., fix sets $X$ and $Y$ that mention up to $k-1$ pigeons and
  such that $X \subseteq Y$. Fix an arbitrary $f \in \{0,1\}^X$. Let
  $A$ and $B$ be the sets of at most $k-1$ pigeons that are mentioned
  in $X$ and $Y$, respectively. Since $X \subseteq Y$ we must have $A
  \subseteq B$. Let $a=|A|$ and $b=|B|$. By construction, the
  assignments $g \in \{0,1\}^Y$ in the support of $\Pi_Y$ are in
  bijective correspondance with the one-to-one mappings $n : B
  \rightarrow [k-1]$, and the same for the $f$ in the support of
  $\Pi_X$ and the one-to-one mappings $m : A \rightarrow
  [k-1]$. Moreover, for each one-to-one mapping $m : A
  \rightarrow [k-1]$, the number of one-to-one mappings $n
  : B \rightarrow [k-1]$ that extend $m$ is
  $\binom{k-1-a}{b-a} (b-a)!$. Thus
  \[ 
  \sum_{g \supseteq f} \Pi_Y(g) = \sum_{n \supseteq m}
  \frac{1}{\binom{k-1}{b} b!} = \frac{\binom{k-1-a}{b-a}
    (b-a)!}{\binom{k-1}{b} b!} = \frac{1}{\binom{k-1}{a} a!} =
  \Pi_X(f).
  \]
  It follows that either $\Pi_X(f) = 0$ and
  $\Pi_X(g) = 0$ for every $g \in \{0,1\}^Y$ such that $g \supseteq
  f$, or $\Pi_X(f) = \sum_{g \supseteq f} \Pi_Y(g)$.  In either case,
  condition 2. is satisfied.
\end{proof}

\subsection{Upper bound for SoS/Lasserre}

We show that $\RPHP(k,n,k-1)$ has a constant-rank Lasserre refutation,
for a constant that is independent of $k$ and $n$. To do that we will
use of following technical identity a couple of times:
\begin{equation} \label{eqn:identity}
\sum_{j \in [n]} \sum_{i \in [n]: i \not= j} \Big(1 - z_i - z_j\Big) z_j
+ (n-2)\sum_{j \in [n]} \Big(z_j^2 - z_j\Big) + \Big({1-\sum_{i \in [n]}
  z_i}\Big)^2 = 1 - \sum_{i \in [n]} z_i.
\end{equation} 
Direct application of this identity shows that the inequality $1 -
\sum_{i \in [n]} x_i \geq 0$ has a rank-2 Lasserre proof from the set
of all inequalities of the form $1 - x_i - x_j \geq 0$ for $i,j \in
[n]$ such that $i \not= j$. This fact should somehow be well-known
since it is a direct consequence of Lemma~1.5 in
\cite{LovaszSchrijver1991Cones}; believe it or not, our argument is a
rewriting of theirs. We use this observation to get a rank-$2$
Lasserre refutation of the pigeonhole principle $\PHP^k_{k-1}$. A
similar proof appears
in~\cite{GrigorievHirschPasechnik2002Complexity}.

\begin{lemma}\label{lem:PHP}
$S(\PHP^k_{k-1})$ has a rank-$2$ Lasserre refutation.
\end{lemma}

\begin{proof}
  Starting at the set of all hole axioms $1 - x_{uw} - x_{vw} \geq 0$
  with a fixed hole $w \in [k-1]$ we get the inequality $1-\sum_{u\in
    [k]} x_{uw} \geq 0$ using~\eqref{eqn:identity}. Adding over all
  holes $w$ we get the inequality $k-1 - \sum_{w \in [k-1]} \sum_{u
    \in [k]} x_{uw} \geq 0$. On the other hand, adding all the pigeon
  axioms $\sum_{w \in [k-1]} x_{uw} - 1 \geq 0$ together we get
  $\sum_{u \in [k]} \sum_{w \in [k-1]} x_{uw} - k \geq 0$. A final
  addition between the two derived inequalities gives $-1 \geq 0$.
\end{proof}

Two more uses of~\eqref{eqn:identity} will help up get a rank-$9$
Lasserre refutation of $\RPHP(k,n,k-1)$ by reduction to
$\PHP^{k}_{k-1}$. The main idea of the proof is to substitute
variables in the proof of $\PHP^{k}_{k-1}$ in Lemma~\ref{lem:PHP} with
polynomials defined on the variables of $\RPHP(k,n,k-1)$.

\begin{lemma}\label{lem:RPHP}
  $S(\RPHP(k,n,k-1))$ has a rank-$9$ Lasserre refutation.
\end{lemma}

\begin{proof}
  Let $S$ be the set of polynomial inequalities in $S(\RPHP(k,n,k-1))$
  and let $x_{u,w}$ be a shorthand for the polynomial $\sum_{\ell \in
    [n]} p_{u,\ell} r_{\ell} q_{\ell,w}$. We want to use the proof of
  the pigeonhole principle in Lemma~\ref{lem:PHP} on the substituted
  variables $ x_{u,v} $, so we need to show how to derive the
  substituted axioms used in that proof.  The inequalities $
  x^{2}_{u,w} -x_{u,w} \geq 0$ are the sum of the following:
\begin{eqnarray}
& & \sum_{\ell \in [n]} \sum_{m \in [n] : m \not= \ell}
(1 - q_{\ell,w} - q_{m,w}) q_{\ell,w} q_{m,w} p_{u,\ell} p_{u,m}
r_\ell r_m \geq 0\\
& & \sum_{\ell \in [n]} \sum_{m \in [n] : m \not= \ell} 
2q_{\ell,w}^2 q_{m,w} p_{u,\ell} p_{u,m} r_\ell r_m \geq 0 \\
& & \sum_{\ell \in [n]} p_{u,\ell}^2 r_\ell^2 q_{\ell,w}^2 \geq 0.
\end{eqnarray}
These have direct rank-$7$ proofs from $S$.
%
% \footnote{There is also a more tricky derivation of
%   small rank for the inequalities $x_{u,w} -x^{2}_{u,w} \geq 0$. The
%   proof in~\ref{lem:PHP} does not use these axioms, so we do not need
%   to show the derivation here.}  
%
The inequalities $\sum_{w \in [k-1]} x_{u,w} - 1 \geq 0$ for $u \in
[k]$ are the sum of the following:
\begin{eqnarray}
& & \sum_{\ell \in [n]} 
\Big(\sum_{w \in [k-1]} q_{\ell,w} - r_\ell \Big) p_{u,\ell} r_{\ell} \geq 0 \\
& & \sum_{\ell \in [n]} \Big(r^{2}_\ell-r_{\ell}\Big) p_{u,\ell} +
\sum_{\ell \in [n]} \Big(r_\ell-p_{u,\ell}\Big) p_{u,\ell} +
\sum_{\ell \in [n]} \Big(p^{2}_{u,\ell}-p_{u,\ell}\Big) \geq 0 \\
& & \sum_{\ell \in [n]} p_{u,\ell} - 1 \geq 0.
\end{eqnarray}
These also have direct proofs from $S$, this time of rank~$3$.  The
inequality $1 - x_{u,w} - x_{v,w} \geq 0$ is the sum of the following:
\begin{eqnarray}
& & \sum_{\ell \in [n]} \Big(1 - p_{u,\ell} - p_{v,\ell}\Big) r_{\ell}
q_{\ell,w} \geq 0 \label{eq:rqvariables1} \\
& & 1-\sum_{\ell \in [n]} r_{\ell} q_{\ell,w} \geq 0. \label{eq:rqvariables2}
\end{eqnarray}
Inequality~\eqref{eq:rqvariables1} has a direct rank-$3$ proof from
$S$.  For~\eqref{eq:rqvariables2} we need to do some more work. Fix
indices $\ell,m \in [n]$ with $\ell \not= m$ and observe that
\begin{eqnarray*}
  \lefteqn{(1 - r_{\ell}q_{\ell,w} - r_{m}q_{m,w})\cdot r_{\ell}q_{\ell,w} = } \\
  & & (3 - r_\ell - r_m - q_{\ell,w} - q_{m,w}) q_{\ell,w} r_{m} q_{m,w} + 
  (q^{2}_{\ell,w} - q_{\ell,w}) r_{m} q_{m,w} + \\  
  & & (q^{2}_{m,w} - q_{m,w}) r_{m} q_{\ell,w} +  
  (r^{2}_{m} - r_{m}) q_{\ell,w} q_{m,w} +  
  (r_{\ell} - r^{2}_{\ell}) q_{\ell,w} + 
  (q_{\ell,w} - q^{2}_{\ell,w}) r^{2}_{\ell}.
\end{eqnarray*}
Note that the first term in the right-hand side of this equation is
the polynomial translation of axiom~\eqref{eq:QinjectiveWide}.  Writing $z_\ell$ for
$r_{\ell} q_{\ell,w}$, this shows that the inequality
$(1-z_\ell-z_\ell) z_\ell \geq 0$ has a rank-$4$ proof from
$S$. Combined with the fact that $z_\ell^2 - z_\ell = (r^2_\ell -
r_\ell) q^2_\ell + (q^2_\ell - q_\ell) r_\ell$,
equation~\eqref{eqn:identity} gives a rank-$4$ proof of $1 -
\sum_{\ell \in [n]} z_\ell \geq 0$. This is
precisely~\eqref{eq:rqvariables2}.

Now we mimic the proof of $\PHP^k_{k-1}$ in Lemma~\ref{lem:PHP}.  For
fixed $w \in [k-1]$, using the derivation of $1 - x_{u,w} - x_{v,w}
\geq 0$ and the derivation of $x_{v,w}^2 - x_{v,w} \geq 0$ in
combination with equation~\eqref{eqn:identity} with $n = k$ and $z_i =
x_{i,w}$ for $i \in [k]$, we get the inequality $1 - \sum_{u \in [k]}
x_{u,w} \geq 0$ by a rank-$9$ proof. Adding all these over $w \in
[k-1]$ gives $k - 1 - \sum_{w \in [k-1]} \sum_{u \in [k]} x_{u,w} \geq
0$.  On the other hand, adding $\sum_{w \in [k-1]} x_{u,w} - 1 \geq 0$
over all $u \in [k]$ gives $\sum_{u \in [k]} \sum_{w \in [k-1]}
x_{u,w} - k \geq 0$. This has a rank-$3$ proof, the rank of the
derivation of $\sum_{w \in [k-1]} x_{u,w} - 1 \geq 0$. A final
addition gives $-1 \geq 0$, all in rank~$9$.
%
% Notice that the proof does not use the
% substituted axioms that have form either $ 1-x_{u,w}\leq 0 $ or $
% x_{u,w}-x^{2}_{u,w} $.
% %
% The proof in Lemma~\ref{lem:PHP} has rank 2: since we can derive
% the substituted axioms in rank 6 and each variable is substituted with a
% polynomial of degree 3, the final proof has rank-12. 
% %
% To get the rank down to 9, we must analyze better the proofs in
% Lemma~\ref{lem:cliqueconstraint} and~\ref{lem:PHP}. In particular the
% latter is just a positive combination of inequalities. Consider the
% ones derived using Lemma~\ref{lem:cliqueconstraint}: in these
% applications of the Lemma, the derivations in
% (\ref{eq:cliqueconstraint}) have of rank 9.
%
\end{proof}


\subsection{Characterization of Sherali-Adams rank}

\aacomment{The characterization below holds also for mentioning-rank
  and the proof is exactly the same (one half of it is already in
  Lemma~\ref{lem:sufficient} and the proof is repeated here). Is it
  worth including this characterization of rank and mentioning-rank
  theorem \`a la Atserias-Dalmau?}

\mlcomment{Maybe it is worth to unify the two cases in a single
  proof. I am not mistaken, it should be possible to define the
  concept of consistent family of distributions for any ``downward
  closed'' set system (i.e.\ a family of sets $ \mathcal{F} $ such
  that for every set $ S \in \mathcal{F} $, all its subsets are in $
  \mathcal{F} $ as well). In particular we obtain a characterization
  of the type: there is a consistent family of distributions with
  respect to a set $ \mathcal{F} $ if and only if there is not
  Sherali-Adams for which the variables in each monomial are in some $
  S \in \mathcal{F} $. The sets of at most $ k $ variables and the
  sets mentioning at most $ k $ pigeons are downward closed, of
  course.}

For a set of polynomial inequalities $S$ on the variables $V$, a
$k$-\emph{consistent family of distributions} is a collection of
probability distributions $\Pi_X$ over assigments $\{0,1\}^X$, as $X$
ranges over the $k$-element subsets of $V$, that satisfies the
following properties:
  \begin{enumerate} \itemsep=0pt
  \item for every set $X$ of up to $k$ variables and every polynomial
    inequality $P \geq 0$ in $S$ that has all its variables in $X$,
    every assignment in the support of $\Pi_X$ satisfies $P \geq 0$,
  \item for every set $X$ of up to $k-1$ variables, every variable $x
    \in V \setminus X$, and every $f \in \{0,1\}^X$ we have $\Pi_X(f)
    = \sum_{g \supseteq f} \Pi_Y(g)$ for $Y = X \cup \{x\}$ and $g$
    ranging over $\{0,1\}^Y$.
  \end{enumerate}
  If such a family of distributions exists we say that $S$ admits a
  $k$-consistent family of distributions.  With this definition, we
  can state the characterization of SA rank as follows:

\begin{theorem}\label{thm:characterization}
Let $F$ be a $k$-CNF. The following are equivalent:
\begin{enumerate} \itemsep=0pt
\item $S(F)$ has an SA-refutation of rank $k$,
\item $S(F)$ does not admit a $k$-consistent family of distributions.
\end{enumerate}
\end{theorem}

We will split the proof of this theorem into two parts that use some
common notation that we define now.  For each monomial $M$, let $X_M$
be the set of the variables in $M$ of non-zero degree and let $a_M$ be
the coefficient of $M$. View each $X_M$ as a new formal variable, and
let $W^k$ denote the collection of all such variables with $|X_M| \leq
k$. For every polynomial $P$ of degree $k$, let $\hat{P}$ be the
linear form on the variables $W^k$ that is obtained from $P$ by
replacing each monomial $M$ by $a_M X_M$. Note that $\hat{P}$ can also
be thought of as a multilinear polynomial on the original variables
$x_1,\ldots,x_n$.  For two disjoint sets of variables $Y$ and $Z$, let
$1_Y 0_Z$ denote the assignment $\{ x \mapsto 1 : x \in Y \} \cup \{ x
\mapsto 0 : x \in Z \}$.

\begin{proof}[Proof of 1. implies 2. in Theorem~\ref{thm:characterization}]
  Let $P_1,\ldots,P_m,P_{m+1},\ldots,P_t$ be the polynomials in an
  SA-refutation of rank $k$ from $S(F)$, where $m$ is the end of the
  phase in which positive linear combinations are not used.  Assuming
  for contradiction that $\{\Pi_X\}$ is a $k$-consistent family, we
  will show that the real assignment $a : W^k \rightarrow \reals$
  defined by
  \[
  a(X) = \Pi_X(1_X)
  \] 
  satisfies $a(\hat{P}_i) \geq 0$ for every $i \in
  \{1,\ldots,m\}$. Since every $\hat{P}_i$ with $i \in
  \{m+1,\ldots,t\}$ is a positive linear combination of the
  inequalities $\hat{P}_\ell$ with $\ell \in \{1,\ldots,m\}$, this
  will show that $a(\hat{P}_i) \geq 0$ for every $i \in
  \{m+1,\ldots,t\}$ and contradict the fact that $P_t = -1$ and hence
  $\hat{P}_t = -1$.

  Let us check that $a$ satisfies every $\hat{P}_i \geq 0$ with $i \in
  \{1,\ldots,m\}$. We prove a stronger claim: if $X_i$ is the set of
  variables in $P_i$ and $\Exp_{X_i}$ denotes expectation under the
  distribution $\Pi_{X_i}$, then $a(\hat{P}_i) = \Exp_{X_i}(P_i)$ and
  every assignment in the support of $\Pi_{X_i}$ satisfies the
  inequality $P_i \geq 0$.  For the first condition, the one stating
  that $a(\hat{P}_i) = \Exp_{X_i}(P_i)$, it suffices to proceed for
  each monomial $M$ in $P$ separately:
  \begin{align*}
  a(\hat{M}) & = c_M a(X_M) = c_M \Pi_{X_M}(1_{M}) = c_M \sum_{g \supseteq
    1_{M}} \Pi_{X_i}(g) = \Exp_{X_i}(M).
  \end{align*}
  The third follows from property 2. in the definition of
  $k$-consistent family and the forth follows from the fact that on
  every assignment in $\{0,1\}^{X_i}$ a monomial with all its
  variables in $X_i$ takes the same value as its multilinear version
  (since $x^2 = x$ on $\{0,1\}$). Adding over all monomials we get
  $a(\hat{P}_i) = \Exp_{X_i}(P_i)$. For the second condition, the one
  stating that every assignment in the support of $\Pi_{X_i}$
  satisfies the inequality $P_i \geq 0$, we proceed by induction on
  $i$.
  
  If $P_i \geq 0$ is a variable-axiom, the claim is obvious since
  every assignment in the support of $\Pi_{X_i}$ gives value $0$ or
  $1$ to the variable. If $P_i = P$ for some inequality $P \geq 0$ in
  $S$, the claim is precisely property 1. in the definition of
  $k$-consistent family. It remains to check the case that $P_i \geq
  0$ is derived from some previous $P_j \geq 0$ with $1 \leq j \leq
  i-1$ by multiplication. Both cases $P_i = x P_j$ and $P_i = (1-x)
  P_j$ have similar proofs, so let us consider the first.  If $x$ does
  not appear in $P_i$ then $P_j=P_i=0$ and the claim is
  obvious. Suppose then that $x$ appears in $P_i$.  For each
  assignment $f$ in the support of $\Pi_{X_i}$ we have either $f(x) =
  0$ or $f(x) = 1$. In the first case, the inequality $xP_j \geq 0$ is
  obviously satisfied. In the second case, the inequality $xP_j \geq
  0$ reduces to $P_j \geq 0$. If $x$ appears in $P_j$, then $X_j =
  X_i$ and $f$ satisfies $P_j \geq 0$ by induction hypothesis. If $x$
  does not appear in $P_j$, let $g$ be the restriction of $f$ to $X_j$
  and observe that, by property 2.  in the definition of
  $k$-consistent family, $g$ is in the support of $\Pi_{X_j}$. By
  induction hypothesis $g$ satisfies $P_j \geq 0$. Since $f \supseteq
  g$ and the variables in $\dom(f) \setminus \dom(g)$ do not appear in
  $P_j$, also $f$ satisfies $P_j \geq 0$, and hence $P_i \geq 0$. This
  concludes the induction and the proof of the lemma.
\end{proof}

\begin{proof}[Proof of 2. implies 1. in Theorem \ref{thm:characterization}]
We prove the contrapositive: we assume the negation 1. and produce a
$k$-consistent family.  Let $P_1 \geq 0,\ldots,P_m \geq 0$ be the
collection of all polynomial inequalities that have an SA-proof of
rank $k$ from $S(F)$. The assumption that 1. fails means that the
corresponding collection of linear forms $\hat{P}_1 \geq 0,
\ldots,\hat{P}_m \geq 0$ on the variables $W^k$ defines a non-empty
polytope $\Pi$ on the hyperplane where the variable $X_1 (=
\emptyset)$ corresponding to the monic monomial of degree zero takes
value $1$. Fix any point $a$ in $\Pi$ such that $a(\emptyset) = 1$
and, for every $X \in W^k$ and $Y \subseteq X$ define $p_X(1_Y
0_{X\setminus Y})$ by the Moebius formula:
\[
p_X(1_Y 0_{X\setminus Y}) = \sum_{Y \subseteq Z \subseteq X}
(-1)^{|Z\setminus Y|} a(Z).
\]
Observe that $p_\emptyset(\emptyset) = a(\emptyset) = 1$.  A useful
observation is that
\begin{equation}
\prod_{x \in Y} x \prod_{x \in X\setminus Y} (1-x) =
\sum_{Y \subseteq Z \subseteq X} (-1)^{|Z\setminus Y|}
\prod_{x \in Z} x. \label{eqn:obs}
\end{equation}
We use this in the following claims:

\begin{claim} $p_X$ is a probability
distribution on $\{0,1\}^X$.
\end{claim}

\begin{proof} 
Since the polynomial in \eqref{eqn:obs} is one of the $P_i$'s, the
linear inequality $\hat{P}_i \geq 0$ is one of the defining
inequalities of $\Pi$ from which we get that $a(\hat{P}_i) \geq 0$ and
hence $p_X(1_Y 0_{X\setminus Y}) \geq 0$. On the other hand we have
\begin{align*} 
\sum_{Y \subseteq X} \sum_{Y \subseteq Z \subseteq X}
(-1)^{|Z\setminus Y|} \prod_{x \in Z} x = \sum_{Y \subseteq X}
\prod_{x \in Y} x \prod_{x \in X \setminus Y} (1-x) = \prod_{x \in
  X}(x + 1 - x) = 1
\end{align*}
from which it follows that
\begin{align*}
\sum_{Y \subseteq X} p_X(1_Y 0_{X\setminus Y}) = \sum_{Y \subseteq X}
\sum_{Y \subseteq Z \subseteq X} (-1)^{|Z\setminus Y|} a(Z) =
a(\emptyset) = 1
\end{align*}
by interpreting each $a(Z)$ as the monic monomial $\prod_{x \in Z} x$.
\end{proof}

\begin{claim} $\{p_X\}_X$ satisfies property 2. in the definition of
$k$-consistent family.
\end{claim}

\begin{proof} This follows from the identity 
$M(Y,Z) = M(Y \cup \{x\},Z) + M(Y,Z\cup \{x\})$.
\end{proof}

\begin{claim} $\{p_X\}_X$ satisfies property 1. in the definition of
$k$-consistent family.
\end{claim}

\begin{proof} 
Fix $X$ and let $C = \bigvee_{x \in Y} \bar{x} \vee \bigvee_{x \in Z}
x$ be a clause in $F$ with $Y \cup Z \subseteq X$. If $Y$ and $Z$ are
not disjoint the claim is obvious.  Assume then that $Y \cap Z =
\emptyset$. By Lemma~\ref{lem:convert}, $-M(Y,Z) \geq 0$ is one of the
$P_i$'s. But then $-M(Y \cup A, Z \cup B) \geq 0$ is also one of the
$P_i$'s for any partition $(A,B)$ of $X \setminus (Y \cup Z)$. From
this we get $p_X(1_{Y \cup A} 0_{Z \cup B}) \leq 0$ for any such
partition. Thus $p_X(f) = 0$ for any $f \in \{0,1\}^X$ that falsifies
$C$.
\end{proof}

This completes the proof of the characterization theorem.
\end{proof}



